Movement- and Traffic-based User Identification in Commercial Virtual Reality Applications: Threats and Opportunities

With the unprecedented diffusion of virtual reality, the number of application scenarios is continuously growing. As commercial and gaming applications become pervasive, the need for the secure and convenient identification of users, often overlooked by the research in immersive media, is becoming more and more pressing. Networked scenarios such as Cloud gaming or cooperative virtual training and teleoperation require both a user-friendly and streamlined experience and user privacy and security. In this work, we investigate the possibility of identifying users from their movement patterns and data traffic traces while playing four commercial games, using a publicly available dataset. If, on the one hand, this paves the way for easy identification and automatic customization of the virtual reality content, it also represents a serious threat to users' privacy due to network analysis-based fingerprinting. Based on this, we analyze the threats and opportunities for virtual reality users' security and privacy.

==> figures/confusion_bts_trf.tex <==
\pgfplotstableread[header=false]{figures/fig_data/confusion_bts_trf_final.dat}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\numrows}{\pgfplotsretval}
\pgfplotstablegetcolsof{\datatable}
\pgfmathtruncatemacro{\numcols}{\pgfplotsretval}
\xdef\LstX{}
\xdef\LstY{}
\xdef\LstC{}
\foreach \Y [evaluate=\Y as \PrevY using {int(\Y-1)},count=\nY] in {1,...,\numrows}
{\pgfmathtruncatemacro{\newY}{\numrows-\Y}
\foreach \X  [evaluate=\X as \PrevX using {int(\X-1)},count=\nX] in {1,...,\numcols}
{
\ReadOutElement{\datatable}{\PrevY}{\PrevX}{\Current}
\pgfmathtruncatemacro{\nZ}{\nX+\nY}
\ifnum\nZ=2
\xdef\LstX{\PrevX}
\xdef\LstY{\PrevY}
\xdef\LstC{\Current}
\else
\xdef\LstX{\LstX,\PrevX}
\xdef\LstY{\LstY,\PrevY}
\xdef\LstC{\LstC,\Current}
\fi
}
}
\edef\temp{\noexpand\pgfplotstableset{
 create on use/x/.style={create col/set list={\LstX}},
 create on use/y/.style={create col/set list={\LstY}},
 create on use/color/.style={create col/set list={\LstC}},}}
\temp
\pgfmathtruncatemacro{\strangenum}{\numrows*\numcols}
\pgfplotstablenew[columns={x,y,color}]{\strangenum}\strangetable

\begin{tikzpicture}
% \pgfplotsset{%
%     colormap={WhiteRedBlack}{%
%         rgb255=(255,255,255)
%         rgb255=(255,0,0)
%         rgb255=(0,0,0)
%     },
% }
\begin{axis}[%
    width=\confwidth,
    height=\confwidth,
    every tick label/.append style={font=\small},
    tick align=outside,
    minor tick num=30,
    xtick pos=left,
ytick pos=left,
    %
    xlabel=Predicted user,
    xlabel near ticks,
    xmin=-0.5, xmax=29.5,
    xtick={0,4,9,14,19,24,29},
    xticklabels={1,5,10,15,20,25,30},
    %
    ylabel=Real user,
    ymin=-0.5, ymax=29.5,
    ytick={0,4,9,14,19,24,29},
    yticklabels={1,5,10,15,20,25,30},
    %
   point meta min=0,
   point meta max=1,
    %
    colorbar,
    colorbar style={ytick={0,0.25,0.5,0.75,1}},
    colormap name=viridis,
    scale mode=scale uniformly,
]
\draw (axis description cs:0,0) -- (axis description cs:1,0);
 \addplot [
        matrix plot,
        %mesh/cols=4,
        point meta=explicit,
] table [meta=color,col sep=comma] \strangetable;
\end{axis}
\end{tikzpicture}

==> figures/confusion_cks_trf.tex <==
\pgfplotstableread[header=false]{figures/fig_data/confusion_cks_trf_final.dat}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\numrows}{\pgfplotsretval}
\pgfplotstablegetcolsof{\datatable}
\pgfmathtruncatemacro{\numcols}{\pgfplotsretval}
\xdef\LstX{}
\xdef\LstY{}
\xdef\LstC{}
\foreach \Y [evaluate=\Y as \PrevY using {int(\Y-1)},count=\nY] in {1,...,\numrows}
{\pgfmathtruncatemacro{\newY}{\numrows-\Y}
\foreach \X  [evaluate=\X as \PrevX using {int(\X-1)},count=\nX] in {1,...,\numcols}
{
\ReadOutElement{\datatable}{\PrevY}{\PrevX}{\Current}
\pgfmathtruncatemacro{\nZ}{\nX+\nY}
\ifnum\nZ=2
\xdef\LstX{\PrevX}
\xdef\LstY{\PrevY}
\xdef\LstC{\Current}
\else
\xdef\LstX{\LstX,\PrevX}
\xdef\LstY{\LstY,\PrevY}
\xdef\LstC{\LstC,\Current}
\fi
}
}
\edef\temp{\noexpand\pgfplotstableset{
 create on use/x/.style={create col/set list={\LstX}},
 create on use/y/.style={create col/set list={\LstY}},
 create on use/color/.style={create col/set list={\LstC}},}}
\temp
\pgfmathtruncatemacro{\strangenum}{\numrows*\numcols}
\pgfplotstablenew[columns={x,y,color}]{\strangenum}\strangetable

\begin{tikzpicture}
% \pgfplotsset{%
%     colormap={WhiteRedBlack}{%
%         rgb255=(255,255,255)
%         rgb255=(255,0,0)
%         rgb255=(0,0,0)
%     },
% }
\begin{axis}[%
    width=\confwidth,
    height=\confwidth,
    every tick label/.append style={font=\small},
    tick align=outside,
    minor tick num=30,
    xtick pos=left,
ytick pos=left,
    %
    xlabel=Predicted user,
    xlabel near ticks,
    xmin=-0.5, xmax=29.5,
    xtick={0,4,9,14,19,24,29},
    xticklabels={1,5,10,15,20,25,30},
    %
    ylabel=Real user,
    ymin=-0.5, ymax=29.5,
    ytick={0,4,9,14,19,24,29},
    yticklabels={1,5,10,15,20,25,30},
    %
   point meta min=0,
   point meta max=1,
    %
    colorbar,
    colorbar style={ytick={0,0.25,0.5,0.75,1}},
    colormap name=viridis,
    scale mode=scale uniformly,
]
\draw (axis description cs:0,0) -- (axis description cs:1,0);
 \addplot [
        matrix plot,
        %mesh/cols=4,
        point meta=explicit,
] table [meta=color,col sep=comma] \strangetable;
\end{axis}
\end{tikzpicture}

==> figures/confusion_fks_trf.tex <==
\pgfplotstableread[header=false]{figures/fig_data/confusion_frk_trf_final.dat}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\numrows}{\pgfplotsretval}
\pgfplotstablegetcolsof{\datatable}
\pgfmathtruncatemacro{\numcols}{\pgfplotsretval}
\xdef\LstX{}
\xdef\LstY{}
\xdef\LstC{}
\foreach \Y [evaluate=\Y as \PrevY using {int(\Y-1)},count=\nY] in {1,...,\numrows}
{\pgfmathtruncatemacro{\newY}{\numrows-\Y}
\foreach \X  [evaluate=\X as \PrevX using {int(\X-1)},count=\nX] in {1,...,\numcols}
{
\ReadOutElement{\datatable}{\PrevY}{\PrevX}{\Current}
\pgfmathtruncatemacro{\nZ}{\nX+\nY}
\ifnum\nZ=2
\xdef\LstX{\PrevX}
\xdef\LstY{\PrevY}
\xdef\LstC{\Current}
\else
\xdef\LstX{\LstX,\PrevX}
\xdef\LstY{\LstY,\PrevY}
\xdef\LstC{\LstC,\Current}
\fi
}
}
\edef\temp{\noexpand\pgfplotstableset{
 create on use/x/.style={create col/set list={\LstX}},
 create on use/y/.style={create col/set list={\LstY}},
 create on use/color/.style={create col/set list={\LstC}},}}
\temp
\pgfmathtruncatemacro{\strangenum}{\numrows*\numcols}
\pgfplotstablenew[columns={x,y,color}]{\strangenum}\strangetable

\begin{tikzpicture}
% \pgfplotsset{%
%     colormap={WhiteRedBlack}{%
%         rgb255=(255,255,255)
%         rgb255=(255,0,0)
%         rgb255=(0,0,0)
%     },
% }
\begin{axis}[%
    width=\confwidth,
    height=\confwidth,
    every tick label/.append style={font=\small},
    tick align=outside,
    minor tick num=30,
    xtick pos=left,
ytick pos=left,
    %
    xlabel=Predicted user,
    xlabel near ticks,
    xmin=-0.5, xmax=29.5,
    xtick={0,4,9,14,19,24,29},
    xticklabels={1,5,10,15,20,25,30},
    %
    ylabel=Real user,
    ymin=-0.5, ymax=29.5,
    ytick={0,4,9,14,19,24,29},
    yticklabels={1,5,10,15,20,25,30},
    %
   point meta min=0,
   point meta max=1,
    %
    colorbar,
    colorbar style={ytick={0,0.25,0.5,0.75,1}},
    colormap name=viridis,
    scale mode=scale uniformly,
]
\draw (axis description cs:0,0) -- (axis description cs:1,0);
 \addplot [
        matrix plot,
        %mesh/cols=4,
        point meta=explicit,
] table [meta=color,col sep=comma] \strangetable;
\end{axis}
\end{tikzpicture}

==> figures/confusion_moh_all.tex <==
\pgfplotstableread[header=false]{figures/fig_data/confusion_moh_all_final.dat}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\numrows}{\pgfplotsretval}
\pgfplotstablegetcolsof{\datatable}
\pgfmathtruncatemacro{\numcols}{\pgfplotsretval}
\xdef\LstX{}
\xdef\LstY{}
\xdef\LstC{}
\foreach \Y [evaluate=\Y as \PrevY using {int(\Y-1)},count=\nY] in {1,...,\numrows}
{\pgfmathtruncatemacro{\newY}{\numrows-\Y}
\foreach \X  [evaluate=\X as \PrevX using {int(\X-1)},count=\nX] in {1,...,\numcols}
{
\ReadOutElement{\datatable}{\PrevY}{\PrevX}{\Current}
\pgfmathtruncatemacro{\nZ}{\nX+\nY}
\ifnum\nZ=2
\xdef\LstX{\PrevX}
\xdef\LstY{\PrevY}
\xdef\LstC{\Current}
\else
\xdef\LstX{\LstX,\PrevX}
\xdef\LstY{\LstY,\PrevY}
\xdef\LstC{\LstC,\Current}
\fi
}
}
\edef\temp{\noexpand\pgfplotstableset{
 create on use/x/.style={create col/set list={\LstX}},
 create on use/y/.style={create col/set list={\LstY}},
 create on use/color/.style={create col/set list={\LstC}},}}
\temp
\pgfmathtruncatemacro{\strangenum}{\numrows*\numcols}
\pgfplotstablenew[columns={x,y,color}]{\strangenum}\strangetable

\begin{tikzpicture}
% \pgfplotsset{%
%     colormap={WhiteRedBlack}{%
%         rgb255=(255,255,255)
%         rgb255=(255,0,0)
%         rgb255=(0,0,0)
%     },
% }
\begin{axis}[%
    width=\confwidth,
    height=\confwidth,
    every tick label/.append style={font=\small},
    tick align=outside,
    minor tick num=30,
    xtick pos=left,
ytick pos=left,
    %
    xlabel=Predicted user,
    xlabel near ticks,
    xmin=-0.5, xmax=29.5,
    xtick={0,4,9,14,19,24,29},
    xticklabels={1,5,10,15,20,25,30},
    %
    ylabel=Real user,
    ymin=-0.5, ymax=29.5,
    ytick={0,4,9,14,19,24,29},
    yticklabels={1,5,10,15,20,25,30},
    %
   point meta min=0,
   point meta max=1,
    %
    colorbar,
    colorbar style={ytick={0,0.25,0.5,0.75,1}},
    colormap name=viridis,
    scale mode=scale uniformly,
]
\draw (axis description cs:0,0) -- (axis description cs:1,0);
 \addplot [
        matrix plot,
        %mesh/cols=4,
        point meta=explicit,
] table [meta=color,col sep=comma] \strangetable;
\end{axis}
\end{tikzpicture}

==> figures/confusion_moh_mov.tex <==
\pgfplotstableread[header=false]{figures/fig_data/confusion_moh_mov_final.dat}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\numrows}{\pgfplotsretval}
\pgfplotstablegetcolsof{\datatable}
\pgfmathtruncatemacro{\numcols}{\pgfplotsretval}
\xdef\LstX{}
\xdef\LstY{}
\xdef\LstC{}
\foreach \Y [evaluate=\Y as \PrevY using {int(\Y-1)},count=\nY] in {1,...,\numrows}
{\pgfmathtruncatemacro{\newY}{\numrows-\Y}
\foreach \X  [evaluate=\X as \PrevX using {int(\X-1)},count=\nX] in {1,...,\numcols}
{
\ReadOutElement{\datatable}{\PrevY}{\PrevX}{\Current}
\pgfmathtruncatemacro{\nZ}{\nX+\nY}
\ifnum\nZ=2
\xdef\LstX{\PrevX}
\xdef\LstY{\PrevY}
\xdef\LstC{\Current}
\else
\xdef\LstX{\LstX,\PrevX}
\xdef\LstY{\LstY,\PrevY}
\xdef\LstC{\LstC,\Current}
\fi
}
}
\edef\temp{\noexpand\pgfplotstableset{
 create on use/x/.style={create col/set list={\LstX}},
 create on use/y/.style={create col/set list={\LstY}},
 create on use/color/.style={create col/set list={\LstC}},}}
\temp
\pgfmathtruncatemacro{\strangenum}{\numrows*\numcols}
\pgfplotstablenew[columns={x,y,color}]{\strangenum}\strangetable

\begin{tikzpicture}
% \pgfplotsset{%
%     colormap={WhiteRedBlack}{%
%         rgb255=(255,255,255)
%         rgb255=(255,0,0)
%         rgb255=(0,0,0)
%     },
% }
\begin{axis}[%
    width=\confwidth,
    height=\confwidth,
    every tick label/.append style={font=\small},
    tick align=outside,
    xtick pos=left,
ytick pos=left,
    minor tick num=30,
    %
    xlabel=Predicted user,
    xlabel near ticks,
    xmin=-0.5, xmax=29.5,
    xtick={0,4,9,14,19,24,29},
    xticklabels={1,5,10,15,20,25,30},
    %
    ylabel=Real user,
    ymin=-0.5, ymax=29.5,
    ytick={0,4,9,14,19,24,29},
    yticklabels={1,5,10,15,20,25,30},
    %
   point meta min=0,
   point meta max=1,
    %
    colorbar,
    colorbar style={ytick={0,0.25,0.5,0.75,1}},
    colormap name=viridis,
    scale mode=scale uniformly,
]
\draw (axis description cs:0,0) -- (axis description cs:1,0);
 \addplot [
        matrix plot,
        %mesh/cols=4,
        point meta=explicit,
] table [meta=color,col sep=comma] \strangetable;
\end{axis}
\end{tikzpicture}

==> figures/confusion_moh_trf.tex <==
\pgfplotstableread[header=false]{figures/fig_data/confusion_moh_trf_final.dat}\datatable
\pgfplotstablegetrowsof{\datatable}
\pgfmathtruncatemacro{\numrows}{\pgfplotsretval}
\pgfplotstablegetcolsof{\datatable}
\pgfmathtruncatemacro{\numcols}{\pgfplotsretval}
\xdef\LstX{}
\xdef\LstY{}
\xdef\LstC{}
\foreach \Y [evaluate=\Y as \PrevY using {int(\Y-1)},count=\nY] in {1,...,\numrows}
{\pgfmathtruncatemacro{\newY}{\numrows-\Y}
\foreach \X  [evaluate=\X as \PrevX using {int(\X-1)},count=\nX] in {1,...,\numcols}
{
\ReadOutElement{\datatable}{\PrevY}{\PrevX}{\Current}
\pgfmathtruncatemacro{\nZ}{\nX+\nY}
\ifnum\nZ=2
\xdef\LstX{\PrevX}
\xdef\LstY{\PrevY}
\xdef\LstC{\Current}
\else
\xdef\LstX{\LstX,\PrevX}
\xdef\LstY{\LstY,\PrevY}
\xdef\LstC{\LstC,\Current}
\fi
}
}
\edef\temp{\noexpand\pgfplotstableset{
 create on use/x/.style={create col/set list={\LstX}},
 create on use/y/.style={create col/set list={\LstY}},
 create on use/color/.style={create col/set list={\LstC}},}}
\temp
\pgfmathtruncatemacro{\strangenum}{\numrows*\numcols}
\pgfplotstablenew[columns={x,y,color}]{\strangenum}\strangetable

\begin{tikzpicture}
% \pgfplotsset{%
%     colormap={WhiteRedBlack}{%
%         rgb255=(255,255,255)
%         rgb255=(255,0,0)
%         rgb255=(0,0,0)
%     },
% }
\begin{axis}[%
    width=\confwidth,
    height=\confwidth,
    every tick label/.append style={font=\small},
    tick align=outside,
    minor tick num=30,
    xtick pos=left,
ytick pos=left,
    %
    xlabel=Predicted user,
    xlabel near ticks,
    xmin=-0.5, xmax=29.5,
    xtick={0,4,9,14,19,24,29},
    xticklabels={1,5,10,15,20,25,30},
    %
    ylabel=Real user,
    ymin=-0.5, ymax=29.5,
    ytick={0,4,9,14,19,24,29},
    yticklabels={1,5,10,15,20,25,30},
    %
   point meta min=0,
   point meta max=1,
    %
    colorbar,
    colorbar style={ytick={0,0.25,0.5,0.75,1}},
    colormap name=viridis,
    scale mode=scale uniformly,
]
\draw (axis description cs:0,0) -- (axis description cs:1,0);
 \addplot [
        matrix plot,
        %mesh/cols=4,
        point meta=explicit,
] table [meta=color,col sep=comma] \strangetable;
\end{axis}
\end{tikzpicture}
